Flickr30k Entities: Collecting Region-to-Phrase Correspondences for Richer Image-to-Sentence Models

The Flickr30k dataset has become a standard benchmark for sentence-based image description. This paper presents Flickr30k Entities, which augments the 158k captions from Flickr30k with 244k coreference chains, linking mentions of the same entities across different captions for the same image, and associating them with 276k manually annotated bounding boxes. Such annotations are essential for continued progress in automatic image description and grounded language understanding. They enable us to define a new benchmark for localization of textual entity mentions in an image. We present a strong baseline for this task that combines an image-text embedding, detectors for common objects, a color classifier, and a bias towards selecting larger objects. While our baseline rivals in accuracy more complex state-of-the-art models, we show that its gains cannot be easily parlayed into improvements on such tasks as image-sentence retrieval, thus underlining the limitations of current methods and the need for further research.

==> commented_out_stuff.tex <==

%\begin{table*}[t]
%\footnotesize
%\begin{center}
%\begin{tabular}{|l|l|c|c|c|c|c|c|c|c|c|c|}
%\hline
%Methods& & bike & boat & car & chair & table & dog & horse & motorcycle & person & overall/mAP\\
%\hline
%\hline
%& \#Instances & { 68 }  & { 27 } & { 59 } & { 25 } & { 65 }  & { 234 } & { 46 } & { 21 } & { 3056 } & { 3601 }\\
%R@100 & {  }  & {  } & {  } & {  } & {  } & { } & {  } & {  } & {  } & {  } & {  }\\
%\hline
%Fast RCNN CCA & R@1 & { 45.59 }  & { 40.74 }& { 55.93 } & { 28.00 } & { 40.00 } & { 73.93 } & { 56.52 } & { 95.24 } & { 63.38 } & { 62.87 }\\
%& R@5 & { 88.24 }  & { 59.26 }& { 77.97 } & { 48.00 } & { 69.23 } & { 90.17 } & { 97.83 } & { 95.24 } & { 84.10 } & { 84.00 }\\
%& R@10 & { 94.12 }  & { 62.96 }& { 79.66 } & { 56.00 } & { 73.85 } & { 90.17 } & { 97.83 } & { 95.24 } & { 87.79 } & { 87.45 }\\
%& R@200 & { 98.53 }  & { 70.37 }& { 86.44 } & { 60.00 } & { 76.92 } & { 91.45 } & { 97.83 } & { 100.00 } & { 94.70 } & { 93.75 }\\
%& AP & { 37.96 }  & { 34.44 }& { 38.94 } & { 18.64 } & { 30.54 } & { 53.87 } & { 57.23 } & { 66.68 } & { 49.88 } & { 43.13 }\\
%\hline
%Fast RCNN Detector & R@1 & { 63.24 }  & { 51.85 }& { 69.49 } & { 24.00 } & { 55.38 } & { 75.21 } & { 65.22 } & { 95.24 } & { 66.75 } & { 66.81 }\\
% & R@5 & { 95.59 }  & { 55.56 }& { 84.75 } & { 44.00 } & { 66.15 } & { 88.89 } & { 95.65 } & { 100.00 } & { 91.33 } & { 87.78 }\\
%& R@10 & { 97.06 }  & { 55.56 }& { 86.44 } & { 52.00 } & { 73.85 } & { 88.89 } & { 95.65 } & { 100.00 } & { 91.33 } & { 90.45 }\\
%& R@200 & { 100.00 }  & { 70.37 }& { 86.44 } & { 72.00 } & { 81.54 } & { 96.58 } & { 97.83 } & { 100.00 } & { 97.05 } & { 96.28 }\\
%& AP & { 62.40 }  & { 40.97 }& { 50.78 } & { 10.43 } & { 47.24 } & { 63.27 } & { 80.04 } & { 73.16 } & { 57.00 } & { 53.92 }\\
%\hline
%\end{tabular}
%\caption{A comparison between the Calibrated CCA model and the Fast RCNN Detector with bounding box regression on phrases which were mapped to PASCAL objects.}
%\label{table:detectorcompare}
%\end{center}
%\end{table*}



%\begin{table*}[t]
%\small
%\begin{center}
%\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
%\hline
%& man & woman & boy & girl & person & people & dog & two men & street & young boy \\
%\hline
%\hline
%\#Instances & { 1093 } & { 597 } & { 139 } & { 135 } & { 132 } & { 116 } & { 112 } & { 105 } & { 101 } & { 94 } \\
%\hline
%AP & { 58.82 } & { 57.76 } & { 61.30 } & { 54.22 } & { 57.03 } & { 28.07 } & { 66.08 } & { 56.72 } & { 34.59 } & { 71.99 }\\
%R@1 & { 72.83 } & { 65.66 } & { 68.35 } & { 64.44 } & { 64.39 } & { 51.72 } & { 70.54 } & { 76.19 } & { 52.48 } & { 78.72 }\\
%R@5 & { 90.30 } & { 93.63 } & { 84.17 } & { 85.93 } & { 85.61 } & { 75.86 } & { 83.04 } & { 89.52 } & { 64.36 } & { 89.36 }\\
%R@10 & { 92.22 } & { 96.15 } & { 85.61 } & { 89.63 } & { 88.64 } & { 81.90 } & { 85.71 } & { 93.33 } & { 69.31 } & { 92.55 }\\
%R@200 & { 96.98 } & { 98.16 } & { 96.40 } & { 97.04 } & { 93.94 } & { 89.66 } & { 91.07 } & { 100.00 } & { 77.23 } & { 95.74 }\\
%\hline
%\hline
%& little girl & child & two people & water & group of people & little boy & table & two women & ball & hat \\
%\hline
%\hline 
%\#Instances  & { 83 } & { 82 } & { 82 } & { 82 } & { 80 } & { 68 } & { 63 } & { 62 } & { 61 } & { 59 } \\
%\hline
%AP & { 66.19 } & { 67.06 } & { 31.51 } & { 29.18 } & { 37.69 } & { 78.51 } & { 46.92 } & { 48.02 } & { 18.33 } & { 33.75 }\\
%R@1  & { 79.52 } & { 78.05} & { 41.46 } & { 47.56 } & { 63.75 } & { 95.59 } & { 58.73 } & { 61.29 } & { 27.87 } & { 40.68 } \\
%R@5 & { 89.16 } & { 92.68 } & { 79.27 } & { 65.85 } & { 86.25 } & { 100.00 } & { 69.84 } & { 93.55 } & { 34.43 } & { 54.24 }\\
%R@10 & { 91.57 } & { 93.90 } & { 89.02 } & { 67.07 } & { 91.25 } & { 100.00 } & { 77.78 } & { 95.16 } & { 36.07 } & { 61.02 }\\
%R@200 & { 95.18 } & { 95.12 } & { 96.34 } & { 73.17 } & { 98.75 } & { 100.00 } & { 85.71 } & { 100.00 } & { 49.18 } & { 69.49 }\\
%\hline
%\end{tabular}
%\vspace{-2mm}
%\caption{ Localization performance for the 24 most common phrases in the test set.}
%\label{table:phraseloc}
%\end{center}
%\end{table*}


\begin{comment}

Table~\ref{table:phraseloc} summarizes the results of our phrase localization experiments, which were designed to provide insight into the following questions:

\begin{enumerate}
%\item How does a CCA embedding handle the long tailed distribution of phrases in Flickr 30k Entities?
\item What effect does using detection-based visual features over classification-based features have on a CCA embedding?
\item How does varying the number of region proposals affect performance of a CCA embedding?
\item What additional visual cues can we leverage to improve performance?
\item How does a CCA embedding perform compared to a detector over common object categories?
\end{enumerate}

%\noindent{\bf Unbalanced Training Data.}  As a first attempt, we train a CCA embedding on the set of all ground-truth phrase-region pairs from the dataset (for phrases associated with multiple regions, we merge them into a single bounding box). The resulting model gets 9.23 mean average precision (mAP) over our phrase types. Part of the reason for the low performance is that the distribution of region counts for different NP chunks in this training set is very unbalanced: a few NP chunks, like {\em a man}, are extremely common, while others, like {\em tattooed, shirtless young man}, occur quite rarely. We found we can alleviate this problem by keeping at most $N$ randomly selected exemplars for each phrase. We get our best mAP of 13.36 by resampling the dataset with $N=10$ (for $N=1$, the mAP is only 8.12). \smallskip

\noindent{\bf Classification vs.\ Detection Features.} Table~\ref{table:phraseloc} (a) and (b) shows the performance of our method with classification-based (ImageNet-trained) and detection-based (PASCAL-fine-tuned) VGG19 features. For comparison, we also list the performance of the weakly supervised method of ~\citet{rohrbach2015} for the same features. While there is a clear intuition that detection-based features should perform better than classification-based features, the magnitude of the difference is not clear a priori.  After all, clothing and body parts, which occurs in almost 70\% of our images, are not among the the PASCAL object classes. While the weakly supervised method of~\citet{rohrbach2015} only achieved a four-point gain in accuracy of the top proposal for each phrase using detection based-features, we achieve a much larger gain of nearly 15 points to having 40.11 mAP with 100 proposals (see Table~\ref{table:phraseloc}(b)). 
\smallskip

\noindent{\bf Number of Object Proposals.} With the much stronger baseline using Fast RCNN features, the number of object proposals is a limiting factor in performance.  With 100 proposals, some phrase types, like people, have an adequate bounding box for almost 90\% of occurrences in the test set, while others, like body parts, have satisfactory bounding boxes in just under 40\% of occurrences.  By doubling the number of proposals to 200, which increases the upper bound performance by eight points, results in less than a one point gain in the accuracy of the top proposal.  Increasing the number of proposals to 500 results in a smaller gain over 100 proposals, but worse performance than ranking 200 proposals.  Increasing the number of proposals to 1,000 or more continues to degrade performance, so we did not include them in the results for this experiment in Table~\ref{table:phraseloc}(b).  Clearly, the CCA embedding, which was trained only on positive data, is not able to leverage the additional proposals to improve performance.
\smallskip

\noindent{\bf Calibrating CCA Scores Between Phrases.} The difference in the mAP over phrase types when compared to over all the unique phrases is also a concern.  Since the difference from the two evaluations is that phrase types groups together similar phrases while the other they are kept separate, it is clear that the relative scores between different phrases are not very comparable.  This is especially an issue if you wish to apply these correspondences to a task like bidirectional retrieval, since it would be difficult to make decisions about similar phrases.  For example, when deciding between two sentences, where one refers to a child as a boy and the other refers to the child as a girl, without having comparable scores between phrases the child could always be marked as one gender simply due to having a better average CCA score for regions.  To help remedy this issue, we also train a sigmoid over phrases that occur more than 30 times in the training set using logistic regression.  For the remaining phrases, we group them by their phrase types and learn a sigmoid over each phrase type.  This results in just over a point improvement in mAP over phrase types as can be seen on the first line of Table~\ref{table:phraseloc}(c).
\smallskip

%\begin{figure*}
%\centering
%\topinset{\large\bfseries(a)}{\includegraphics[height=4cm]{Figures/detectorRat1.png}}{0in}{-1.5in}
%\hspace{0.7cm}\topinset{\large\bfseries(b)}{\includegraphics[height=4cm]{Figures/detectorAP.png}}{0in}{-1.5in}
%\caption{Comparison over phrase types showing how averaging the CCA score for a region-phrase correspondence the output of the Fast RCNN detector affects performance.}
%\label{fig:pascalTypes}
%\end{figure*}
\end{comment}


\begin{table*}
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\hline
 & people &  clothing & bodyparts & animals & vehicles  & instruments & scene & other \\
\hline
\hline
\#Instances & { 5,656 }  & { 2,306 } & { 523 } & { 518 } & { 400 }  & { 162 } & { 1,619 } & { 3,374 }\\
\hline
%Calibrated CCA&AP & { 32.95 }  & { 24.03 } & { 13.24 } & { 35.43 } & { 36.29  } & { 19.69 } & { 21.49 } & { 15.46 }\\
%+Size+Color&R@1 & { 61.97 } & { 45.06 }  & { 16.25 }& { 65.83 } & { 66.50 } & { 37.65 } & { 50.40 } & { 30.85 } \\
%&R@5 & { 83.47 }  & { 64.74 }& { 29.25 } & { 81.08 } & { 88.00 } & { 53.70 } & { 69.55 } & { 53.44 } \\
%&R@10 & { 87.84 }  & { 69.60 }& { 34.23 } & { 83.59 } & { 90.00 } & { 62.96 } & { 73.50 } & { 59.90 }\\
%&R@200 & { 95.31 }  & { 77.36 } & { 50.48 } & { 89.58 } & { 94.25 } & { 80.86 } & { 83.01 } & { 75.70 }\\
%\hline

%AP & { 44.29 } & { 24.03 } & { 13.24 } & { 39.04 } & { 45.72  } & { 19.69 } & { 24.15 } & { 15.99 }\\
%R@1 & { 65.28 } & { 45.06 }  & { 16.25 } & { 66.41 } & { 70.50 } & { 37.65 } & { 50.65 } & { 31.15 }\\
%R@5 & { 86.10 } & { 64.74 } & { 29.25 } & { 80.31 } & { 88.25 } & { 53.70 } & { 69.55 } & { 53.44 }\\
%R@10 & { 90.03 } & { 69.60 } & { 34.23 } & { 83.98 } & { 90.25 } & { 62.96 } & { 73.50 } & { 59.96 }\\
R@1 CCA & { 61.24 } & { 36.90 } & { 15.30} & { 62.74 } & { 59.75 } & { 31.48 } & { 31.93 } & { 25.34 }\\
R@1 CCA+Size & { 64.73 } & { 39.20 } & { 15.49 } & { 64.09 } & { 67.75 } & { 37.65 } & { 51.33 } & { 30.50 }\\
R@1 CCA+Size+Color & { 64.73 } & { 46.88 } & { 17.21 } & { 65.83 } & { 68.75 } & { 37.65 } & { 51.39 } & { 31.77 }\\
R@200 & { 96.52 } & { 77.36 } & { 50.48 } & { 91.12 } & { 94.50 } & { 80.86 } & { 83.01 } & { 75.87 }\\
\hline
AP CCA & { 40.51 } & { 20.19 } & { 9.30 } & { 45.52 } & { 37.84 } & { 15.73 } & { 15.21 } & { 14.58 }\\
AP CCA+Size & { 44.52 } & { 21.10 } & { 8.86 } & { 47.02 } & { 43.40 } & { 21.53 } & { 23.94 } & { 15.74 }\\
AP CCA+Size+Color & { 44.52 } & { 24.50 } & { 13.50 } & { 47.97 } & { 44.36 } & { 20.72 } & { 24.15 } & { 16.04 }\\
\hline
\end{tabular}
\caption{Localization performance over phrase types using our Avg CCA and Fast RCNN Detector+Size+Color model to rank 200 object proposals per image. We report average precision (AP) and Recall@$K$ (see Section~\ref{sec:textToImageReference} for details).}
\label{table:phraseLocBreakdown}
\end{center}
\end{table*}


%\noindent {\bf Color and Size Preference.} The first example in Figure~\ref{fig:Examples} describes a man with an orange hat.  Despite not being the only person in the picture, he clearly is the center of attention and takes up a larger share of the image than any of the other people in the background. This preference towards describing the larger objects when multiple instances occur within an image can be leveraged to further improve performance on our text-to-image reference task.  
% Some object types, like body parts, which on average only take up 8\% of an image compared to scene terms which take up 48\% of an image on average, may have less of a preference towards larger objects than others.  This leads us to define a combined score



\begin{comment}
\begin{table*}
\begin{center}
\caption{R@1 performance over phrases that mention a color in the test set.  We also include R@200, which provides an upper bound performance of the different colors.  See Section~\ref{sec:color} for details.}
\label{table:colorloc}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
 & black & red & blue & white & green & yellow & brown & orange & pink & grey & purple & overall\\
\hline
\hline
\#Instances & { 312 } & { 296 } & { 295 } & { 267 } & { 155 }  & { 154 } & { 112 } & { 88 } & { 79 } & { 71 } & { 23 } & { 1852 }\\
\hline
Color SVM & { 10.90 } & { 6.42 } & { 8.47 } & { 10.49 } & { 8.39 } & { 1.30 } & { 38.39 } & { 13.64 } & { 7.59 } & { 12.68 } & { 0 } & { 10.31 }\\
Color Fast RCNN & { 36.22 } & { 60.14 } & { 52.88 } & { 50.56 } & { 56.77 } & { 49.35 } & { 57.14 } & { 56.82 } & { 48.10 } & { 57.75 } & { 47.83 } & { 49.24 }\\
\hline
CCA (Fast RCNN) & { 37.82 } & { 41.55 } & { 40.34 } & { 42.70 } & { 39.35 } & { 33.77 } & { 56.25 } & { 47.73 } & { 29.11 } & { 36.62 } & { 39.13 } & { 40.50 }\\
{ +Color Fast RCNN} & { 51.92 }  & { 63.18 } & { 56.25 } & { 55.06 } & { 58.71 } & { 51.95 } & { 62.50 } & { 60.23 } & { 54.43 } & { 60.56 } & { 56.52 } & { 57.18 }\\
\hline
R@200 & { 82.69 } & { 84.80 } & { 81.36 } & { 82.40 } & { 82.58 } & { 83.77 } & { 88.39 } & { 80.68 } & { 74.68 } & { 80.28 } & { 82.61 } & { 82.67 }\\
\hline
\end{tabular}
\end{center}
\end{table*}
\end{comment}




%\begin{table*}
%\caption{Comparison of related datasets.}
%\label{table:dataCompare}
%\centering
%\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
%\hline
%& \multicolumn{4}{|c|}{Image-Phrase Datasets} & \multicolumn{2}{|c|}{Image-Sentence Datasets}\\
%\hline
%Dataset & Scene Graph & Visual Genome\textsuperscript{*} & ReferIt & Google Refexp & MSCOCO & Flickr30k Entities\\
%& \parbox{0.1\linewidth}{\citep{Johnson2015CVPR}} & \parbox{0.1\linewidth}{\citep{krishnavisualgenome}} & \parbox{0.1\linewidth}{\citep{kazemzadeh-EtAl:2014:EMNLP2014}} & \citep{mao2015generation} & \citep{lin2014microsoft} & \\
%\hline
% 5,000 & 108,077 & 19,894 & 26,711 & 328,000 & 31,783\\
% & 18.8 & Approx 56 & 4.9 & 2.1 & 7.7 & 8.7\\
% 6,745 & 110,689 & 238 & 80 & 91 & 44,518\\
% & 13.9 & Approx. 54 & 406.1 & 685.3 & 27472.5 & 6.2\\
% & -- & -- & -- & -- & 5 & 5\\
% & 33.0 & 40 & 6.6 & 3.9 & -- & --\\
%\hline
%\end{tabular}
%\vspace{-3mm}
%\flushleft\hspace{1mm}\begingroup
%    \fontsize{6pt}{6pt}\selectfont
% *obtained via personal communication with the authors
%\endgroup
%\vspace{-3mm}
%\end{table*}


%\begin{figure}
%\centering
%\includegraphics[width=0.4\textwidth]%{Figures/entityVerifyResults.png}
%\caption{}
%\label{fig:}
%\end{figure}

